A Unifying Complexity Certification Framework for Active-Set Methods for Convex Quadratic Programming

In model predictive control (MPC) an optimization problem has to be solved at each time step, which in real-time applications makes it important to solve these optimization problems efficiently and to have good upper bounds on worst-case solution time. Often for linear MPC problems, the optimization problem in question is a quadratic program (QP) that depends on parameters such as system states and reference signals. A popular class of methods for solving such QPs is active-set methods, where a sequence of linear systems of equations is solved. We propose an algorithm for computing which sequence of subproblems an active-set algorithm will solve, for every parameter of interest. By knowing these sequences, a worst-case bound on how many iterations, and ultimately the maximum time, the active-set algorithm requires to converge can be determined. The usefulness of the proposed method is illustrated on a set of QPs, originating from MPC problems, by computing the exact worst-case number of iterations primal and dual active-set algorithms require to reach optimality.

==> alg/cert_algorithm.tex <==
\begin{algorithm}[H]
  \caption{Partition state space based on active-set changes}\label{alg:main}
  \begin{algorithmic}[1]
	\Require $\Theta_0, \mathcal{A}_0, F_0, G_0,$ mpQP 
	\Ensure FinalPartition
	\State Push $(\Theta_{0}, \mathcal{A}_0,F_0,G_0,\text{false},\text{false},0,\text{NaN})$ to $S$
  \While {$S$ is not empty}
  \State Pop $p_c$ from $S$
  \If {$p_c$ local optimum}
  \State Partition = RemoveConstraint($p_c$,mpQP)
  \Else
  \State Partition = AddConstraint($p_c$, mpQP)
  \EndIf
  \For {$p$ in Partition}
  \If {$p$ is global optimum}
  \State Append $p$ to FinalPartition
  \Else 
  \State push $p$ to $S$
  \EndIf
  \EndFor
  \EndWhile
  \State \Return FinalPartition
  \end{algorithmic}
\end{algorithm}


==> alg/primal_algorithm.tex <==
\begin{algorithm}[H]
  \caption{Primal Active-Set Method for QP \cite{nocedal}}\label{alg:primal-as}
  \begin{algorithmic}[1]
	\Require $x_0, \mathcal{W}_0, k=1$
	\Ensure $x_k^*, \lambda_k, \mathcal{W}_k $
	\While {true}
	\State Compute $x_k^*$ and $\lambda_k$ by solving \eqref{eq:kkt} 
  \State $p_k \leftarrow x^*_k - x_k$
  \If{$p_k = 0$}
  	\If{$\lambda_k \geq 0$}
	\Return $x_k^*, \lambda_k , \mathcal{W}_k$  
	\Else \quad $l \leftarrow \underset{i\in \mathcal{W}_k }{\text{argmin }} [\lambda_k]_i$,
	\: $\mathcal{W}_{k+1} \leftarrow \mathcal{W}_k\setminus\{l\}$ \label{line:const-rm}
  \EndIf
  \Else 
  \State $m \leftarrow \underset{i \in \mathcal{C}^+_k}{\text{argmin }} \alpha^i_k$,  \: $\alpha_k \leftarrow \min\{1,\alpha^m_k\}$
  \If{$\alpha_k< 1$} \: $\mathcal{W}_{k+1}  \leftarrow \mathcal{W}_k \cup \{m\}$  
\EndIf
  \State $x_{k+1} \leftarrow x_k + \alpha_k p_k$
\EndIf
	\State $k \leftarrow k +1$
  \EndWhile
  \end{algorithmic}
\end{algorithm}


==> alg/primal_algorithm2.tex <==
\begin{algorithm}[H]
  \caption{Primal Active-Set Method for QP \cite{nocedal}}\label{alg:primal-as}
  \begin{algorithmic}[1]
	\Require $x_0, \mathcal{A}_0, k=1$
	\Ensure $x_k^*, \lambda_k, \mathcal{A}_k $
	\While {true}
	\State Compute $x_k^*$ and $\lambda_k$ by solving \eqref{eq:kkt} 
  \State $p_k \leftarrow x^*_k - x_k$
  \If{$p_k = 0$}
  	\If{$\lambda_k \geq 0$}
	\Return $x_k^*, \lambda_k , \mathcal{A}_k$  
	\Else \quad $l \leftarrow \underset{i\in \mathcal{A}_k }{\text{argmin }} [\lambda_k]_i$,
\: $\mathcal{A}_{k+1} \leftarrow \mathcal{A}_k\setminus\{l\}$
  \EndIf
  \Else 
  \State $m \leftarrow \underset{i \in \mathcal{I}_k,\: [A]_i p_k > 0 }{\text{argmin}} \frac{[b]_i - [A]_i x_k}{[A]_i p_k}$ 
  \State $\alpha_k \leftarrow \min\{1,\frac{[b]_m-[A]_m x_k}{[A]_m p_k}\}$, \:$x_{k+1} \leftarrow x_k + \alpha_k p_k$
  \If{$\alpha_k< 1$} \: $\mathcal{A}_{k+1}  \leftarrow \mathcal{A}_k \cup \{m\}$  
\EndIf
\EndIf
	\State $k \leftarrow k +1$
  \EndWhile
  \end{algorithmic}
\end{algorithm}


==> alg/primal_algorithm_alternative.tex <==
\begin{algorithm}[H]
  \caption{Primal Active-Set Method for QP \cite{nocedal}}\label{alg:primal-as}
  \begin{algorithmic}[1]
	\Require $x_0, \mathcal{W}_0, k=1$
	\Ensure $x_k^*, \lambda_k, \mathcal{W}_k $
	\While {true}
	\State Compute $x_k^*$ and $\lambda_k$ by solving \eqref{eq:kkt} 
  \State $p_k \leftarrow x^*_k - x_k$
  \If{$A x^*_k \leq b + W\theta$}
  	\If{$\lambda_k \geq 0$}
	\Return $x_k^*, \lambda_k , \mathcal{W}_k$  
	\Else \quad $l \leftarrow \underset{i\in \mathcal{W}_k }{\text{argmin }} [\lambda_k]_i$,
	\: $\mathcal{W}_{k+1} \leftarrow \mathcal{W}_k\setminus\{l\}$ \label{line:const-rm}
	\State \quad $x_{k+1} \leftarrow  x_k^*$
  \EndIf
  \Else\quad $m \leftarrow \underset{i \in \mathcal{C}^+_k}{\text{argmin }} \alpha^i_k,\quad \mathcal{W}_{k+1}  \leftarrow \mathcal{W}_k \cup \{m\}$  
  \State \quad $x_{k+1} \leftarrow x_k + \alpha_k p_k$
\EndIf
	\State $k \leftarrow k +1$
  \EndWhile
  \end{algorithmic}
\end{algorithm}


==> alg/stationary-alg.tex <==
\begin{algorithm}[H]
  \caption{Check if a region has reached local optimality}
  \label{alg:stationary}
  \begin{algorithmic}[1]
	\State \textsc{isLocallyOptimal}{($(\Theta,\mathcal{W},F,G,s, k, \hat{n})$, mpQP)}
	%\Require $(\Theta,\mathcal{A},F,G,s, k, \hat{p})$ , mpQP
	%\Ensure $isstationary$
	\State Compute $F^*$ and $G^*$ according to \eqref{eq:F-star}
	\If{$s==1$} \Return \texttt{true}
  \EndIf
  \If{Case 1} \Return $\tilde\pi_k p_0 == 0$
  \Else \text{ }\Return $(F^*== F \textbf{ and } G^*==G)$ 
  \EndIf 
  \end{algorithmic}
\end{algorithm}


==> sec/check_stationarity.tex <==
If a full step was taken in the previous iteration, the next iterate will be a locally optimal point. However, there are cases when a local optimum is reached without a full step being taken in the previous iteration. To detect these cases, $p_k=0$, or equivalently $x^*_k = x_k$, has to be checked explicitly. As has been discussed in Section \ref{ssec:add}, the iterates will not necessarily be affine in the parameter, and the same can be said about the search direction $p_k$. Thus, the analysis is split into the same two cases as before. 

From Corollary \ref{prop:add-col} it follows that  $\tilde H^*_k H p_0 = 0\Rightarrow p_k = 0$ in Case 1. Hence, the region is locally optimal if $\tilde H^*_k H p_0 = 0$.

The affine structure in Case 2 simply means that $F^*_k = F_k$ and $G^*_k = G_k$ give $x^*_k=x_k$.



==> sec/ex_gen_mpqp_single.tex <==
\begin{figure}
  \centering
  \input{fig/iter-bar.tex}\newline
  \begin{subfigure}[b]{0.25\textwidth}
	\begin{tikzpicture}
	  \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=0.95\textwidth]{fig/quad-ex.eps}};
	  \begin{scope}[x={(image.south east)},y={(image.north west)}]
	  \node (xlabel) at (0.5,0.05) {$\theta_1$};
	  \node (xmintick) at (0.155,0.05) {$0$};
	  \node (xmaxtick) at (0.875,0.06) {$1$};
	  \node (ylabel) at (0.085,0.5) {$\theta_2$};
	  \node[align=right] (ymintick) at (0.09,0.15) {$0$};
	  \node[align=right] (ymaxtick) at (0.09,0.85) {$1$};
	  \node (dummy) at(-0.025,0.5){};
	\end{scope}
  \end{tikzpicture}
	\caption{Contrived mpQP, $p=2$}
	\label{fig:genmpqp}
  \end{subfigure}
  \begin{subfigure}[b]{0.25\textwidth}
	\begin{tikzpicture}
	  \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=0.95\textwidth]{fig/dblint-clean.eps}};
	  \begin{scope}[x={(image.south east)},y={(image.north west)}]
	  \node (xlabel) at (0.5,0.05) {$\theta_1$};
	  \node (xmintick) at (0.155,0.05) {$\text{-}1.5$};
	  \node (xmaxtick) at (0.875,0.06) {$1.5$};
	  \node (ylabel) at (0.085,0.5) {$\theta_2$};
	  \node[align=right] (ymintick) at (0.075,0.15) {$\text{-}1$};
	  \node[align=right] (ymaxtick) at (0.09,0.85) {$1$};
	  \node (dummy) at(-0.025,0.5){};
	\end{scope}
  \end{tikzpicture}
	\caption{Double integrator, $p=4$}
	\label{fig:dbint}
  \end{subfigure}
  \begin{subfigure}[b]{0.25\textwidth}
	\begin{tikzpicture}
	  \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=0.95\textwidth]{fig/dc-motor.eps}};
	  \begin{scope}[x={(image.south east)},y={(image.north west)}]
	  \node (xlabel) at (0.5,0.05) {$\theta_1$};
	  \node (xmintick) at (0.125,0.05) {$\text{-}0.15$};
	  \node (xmaxtick) at (0.875,0.06) {$0.15$};
	  \node (ylabel) at (0.085,0.5) {$\theta_2$};
	  \node[align=right] (ymintick) at (0.08,0.15) {$\text{-}1$};
	  \node[align=right] (ymaxtick) at (0.095,0.85) {$1$};
	  \node (dummy) at(-0.025,0.5){};
	\end{scope}
  \end{tikzpicture}
  \caption{DC-motor, $p=6$}
	\label{fig:dcmotor}
  \end{subfigure}
  \begin{subfigure}[b]{0.25\textwidth}
	\begin{tikzpicture}
	  \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=0.95\textwidth]{fig/invpend-clean.eps}};
	  \begin{scope}[x={(image.south east)},y={(image.north west)}]
	  \node (xlabel) at (0.5,0.05) {$\theta_1$};
	  \node (xmintick) at (0.125,0.05) {$\text{-}20$};
	  \node (xmaxtick) at (0.875,0.06) {$20$};
	  \node (ylabel) at (0.085,0.5) {$\theta_2$};
	  \node[align=right] (ymintick) at (0.045,0.15) {$\text{-}20$};
	  \node[align=right] (ymaxtick) at (0.07,0.85) {$20$};
	  \node (dummy) at(-0.025,0.5){};
	\end{scope}
  \end{tikzpicture}
  \caption{Inverted pendulum, $p=8$}
	\label{fig:invpend}
  \end{subfigure}
  \begin{subfigure}[b]{0.25\textwidth}
	\begin{tikzpicture}
	  \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=0.95\textwidth]{fig/nonlindemo-clean.eps}};
	  \begin{scope}[x={(image.south east)},y={(image.north west)}]
	  \node (xlabel) at (0.5,0.05) {$\theta_1$};
	  \node (xmintick) at (0.125,0.05) {$\text{-}0.5$};
	  \node (xmaxtick) at (0.875,0.06) {$2$};
	  \node (ylabel) at (0.085,0.5) {$\theta_2$};
	  \node[align=right] (ymintick) at (0.045,0.15) {$\text{-}0.5$};
	  \node[align=right] (ymaxtick) at (0.095,0.85) {$1$};
	  \node (dummy) at(-0.025,0.5){};
	\end{scope}
  \end{tikzpicture}
  \caption{Nonlinear demo, $p=10$}
	\label{fig:nonlin}
  \end{subfigure}
  \begin{subfigure}[b]{0.25\textwidth}
	\begin{tikzpicture}
	  \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=0.95\textwidth]{fig/air-clean.eps}};
	  \begin{scope}[x={(image.south east)},y={(image.north west)}]
	  \node (xlabel) at (0.5,0.05) {$\theta_1$};
	  \node (xmintick) at (0.125,0.05) {$\text{-}20$};
	  \node (xmaxtick) at (0.875,0.06) {$20$};
	  \node (ylabel) at (0.085,0.5) {$\theta_2$};
	  \node[align=right] (ymintick) at (0.07,0.15) {$\text{-}20$};
	  \node[align=right] (ymaxtick) at (0.07,0.85) {$20$};
	  \node (dummy) at(-0.025,0.5){};
	\end{scope}
  \end{tikzpicture}
  \caption{ATFI-16, $p=10$}
	\label{fig:ATFI-16}
  \end{subfigure}
  \caption{2D-slice of the resulting parameter regions with ${\theta_i = 0,\: i>2}$, produced by Algorithm \ref{alg:main} for the primal problems. The same color means same number of QP iterations.}\label{fig:iterfig}

   
\end{figure}


==> sec/ex_inv_pend.tex <==
Inverted pendulum from MATLAB toolbox...
The same example is considered in \cite{10.1109TAC.2017.2696742} where the GI algorithm is certified.


==> sec/ex_overlap.tex <==
%\begin{figure}[htpb]
%  \centering
%  \includegraphics[width=0.75\linewidth]{fig/servo.eps}
%  \caption{Servomotor}
%  \label{fig:fig/servo}
%\end{figure}
%\begin{figure}[htpb]
%  \centering
%  \includegraphics[width=0.5\linewidth]{fig/inv_pend.eps}
%  \caption{Inverted pendulum}
%  \label{fig:fig/inv_pend}
%\end{figure}
%
%\begin{figure}[htpb]
%  \centering
%  \includegraphics[width=0.5\linewidth]{fig/non-lin.eps}
%  \caption{Inverted pendulum}
%  \label{fig:fig/inv_pend}
%\end{figure}
\begin{figure}
  \centering
  \input{fig/iter-bar.tex}
  \begin{subfigure}[b]{0.23\textwidth}
%	\includegraphics[width=\textwidth]{fig/genmpqp.eps}
	\begin{tikzpicture}
	  \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=\textwidth]{fig/quad-ex-overlap}};
	  \begin{scope}[x={(image.south east)},y={(image.north west)}]
		%\draw[red,ultra thick,rounded corners] (0.62,0.65) rectangle (0.78,0.75);
	  \node (xlabel) at (0.5,0.05) {$\theta_1$};
	  \node (xmintick) at (0.155,0.05) {$0$};
	  \node (xmaxtick) at (0.875,0.06) {$1$};
	  \node (ylabel) at (0.085,0.5) {$\theta_2$};
	  \node[align=right] (ymintick) at (0.095,0.15) {$0$};
	  \node[align=right] (ymaxtick) at (0.095,0.85) {$1$};
	  \node (dummy) at(-0.025,0.5){};
	\end{scope}
  \end{tikzpicture}
	\caption{General mpQP, $p=2$}
	\label{fig:genmpqp}
  \end{subfigure}
  \begin{subfigure}[b]{0.23\textwidth}
	%\includegraphics[width=\textwidth]{fig/doubleint.eps}
	\begin{tikzpicture}
	  \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=0.95\textwidth]{fig/dc-motor-overlap.eps}};
	  \begin{scope}[x={(image.south east)},y={(image.north west)}]
		%\draw[red,ultra thick,rounded corners] (0.62,0.65) rectangle (0.78,0.75);
	  \node (xlabel) at (0.5,0.05) {$\theta_1$};
	  \node (xmintick) at (0.155,0.05) {$\text{-}1.5$};
	  \node (xmaxtick) at (0.875,0.06) {$1.5$};
	  \node (ylabel) at (0.085,0.5) {$\theta_2$};
	  \node[align=right] (ymintick) at (0.075,0.15) {$\text{-}1$};
	  \node[align=right] (ymaxtick) at (0.09,0.85) {$1$};
	  \node (dummy) at(-0.025,0.5){};
	\end{scope}
  \end{tikzpicture}
	\caption{Double integrator, $p=4$}
	\label{fig:dbint}
  \end{subfigure}
  \caption{Resulting partition when quadratic inequalties are relaxed according to Section \ref{}.}\label{fig:overlapfig}

   
\end{figure}

